Pooling Image Datasets With Multiple Covariate Shift and Imbalance

Small sample sizes are common in many disciplines, which necessitates pooling roughly similar datasets across multiple institutions to study weak but relevant associations between images and disease outcomes. Such data often manifest shift/imbalance in covariates (i.e., secondary non-imaging data). Controlling for such nuisance variables is common within standard statistical analysis, but the ideas do not directly apply to overparameterized models. Consequently, recent work has shown how strategies from invariant representation learning provides a meaningful starting point, but the current repertoire of methods is limited to accounting for shifts/imbalances in just a couple of covariates at a time. In this paper, we show how viewing this problem from the perspective of Category theory provides a simple and effective solution that completely avoids elaborate multi-stage training pipelines that would otherwise be needed. We show the effectiveness of this approach via extensive experiments on real datasets. Further, we discuss how this style of formulation offers a unified perspective on at least 5+ distinct problem settings, from self-supervised learning to matching problems in 3D reconstruction.

==> sections/proof_of_concept.tex <==




==> sections/test.tex <==






Assume we map our images to a latent space in a way that it preserves the structure, i.e. it is equivariant to specific characteristics. These characteristics can be either discrete (e.g. gender) or continuous (e.g. age) which are quantized. We denote the autoencoder $(F, F^{-1})$ since it corresponds to a pair of functors.

Assume the morphisms in the latent space are linear transformations $W\in\mathbb{R}^{n\times n}$. That design choice provides the following capabilities:
\begin{itemize}
    \item Smooth image interpolation: Assume we have two images $I_1, I_2$ for which it holds $F(I_1)^TW = F(W_2)$ (i.e. the are connected with a morphism in the latent space). Then we can generate all the ``intermediate'' images by taking $F^{-1}(F(I_1)^TW^{\alpha}),\ \alpha\in[0,1]$.
    
    \item Effect generalization: Assume $W$ represent the increase of the age by 10 years. By continuously applying $W$ to a latent vector, we can get images of an older person that may be beyond the examples seen during training (similarly to rotations and scaling in the MNIST example).
    
    \item Composition of effects: We can compose multiple effects according to $W_1 \circ W_2 = W_1 \times W_2$ and generate images that are not seen during training.
\end{itemize}

Current models have the following limitations that we address:
\begin{itemize}
    \item Image interpolation for multiple effects. Many works focus on interpolating between two classes of images (e.g. young and old) but the generalization to a model that can handle multiple interpolations is not clear.
    \item Generalization between seen examples: Many works, although can perform interpolation for multiple effects, they are restricted to the range in betwwen two well-defined (during training) classes of data (e.g. young and old). Taking an image of an old person and ``making him even older'' is not working in such models.
    \item Capturing continuous effects: Most works focus on discrete effects (e.g. smiling, gender, etc.) and they do not provide a way to address continuous effects such as hair length, age, etc.
\end{itemize}
The main difference is that other works try to map the images to a nice manifold in which e.g. linear interpolation can work. In contrast, we learn the interpolation function. While there are some works that try to do that, they do it in a way that we can not generalize beyond the seen images or perform interpolation for continuous effects (e.g. age). We address that by using a linear transformation instead of a complicated NN.
